Identifying Breakdowns in Conversational Recommender Systems using User Simulation

We present a methodology to systematically test conversational recommender systems with regards to conversational breakdowns. It involves examining conversations generated between the system and simulated users for a set of pre-defined breakdown types, extracting responsible conversational paths, and characterizing them in terms of the underlying dialogue intents. User simulation offers the advantages of simplicity, cost-effectiveness, and time efficiency for obtaining conversations where potential breakdowns can be identified. The proposed methodology can be used as diagnostic tool as well as a development tool to improve conversational recommendation systems. We apply our methodology in a case study with an existing conversational recommender system and user simulator, demonstrating that with just a few iterations, we can make the system more robust to conversational breakdowns.

==> cui2024-crs-breakdowns-07.tex <==
\section{Summary per failure for first iteration}

\subsection{System failure}

\begin{table}
	\centering
	\caption{System failure summary. The sign + is used to represent utterance with more than one intent.}
	\begin{tabularx}{\linewidth}{X|c}
		Sequence of intents &  Count \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL') & 5 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_ELICIT', 'U\_REVEAL') & 2 \\ \hline
		\hline
		Total & 13 \\ \hline
	\end{tabularx}
\end{table}

\subsection{Flow discontinuation}

\begin{table}
	\centering
	\caption{Flow discontinuation summary.}
	\begin{tabularx}{\linewidth}{X|c}
		Sequence of intents &  Count \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM')                                                                                                         &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM')                                                                                                                                                  &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS')                                                                                                                                                           &       9 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT')                                                                                                                                                                          &       3 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL')                                                                                              &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY')                                                                                                                                    &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL')                                                                                                                                                  &       5 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY')                                                                                                                        &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL')                                                                                                                                                                                             &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP')                                                                                                                                                            &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM')                                                                                                                                                                                                                     &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND')                                                                                                                                                                                    &       3 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL')                                                                                                                                                                                                                     &      11 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REMOVE\_PREFERENCE')                                                                                                                                       &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_NO\_RESULTS')                                                                                                                                  &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM')                                                                                                                         &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL')                                                                                                                                                                                                                                             &       4 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL')                                                                                                                                                                           &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE')                                                                                                                                 &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE')                                                                                                                                                                                                 &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP')                                                                                                                                           &       3 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM')                                                                       &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE')                                                                                                                                                               &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_ELICIT')                                                                                                                                                                                                                                  &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS')                                                                                                                                                                                   &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP')                                                                                                                                          &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM')                                                                                                                                                                                                                                 &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_CONTINUE\_RECOMMENDATION')                                                                                                                                         &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM')                                                                                                                                                              &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP')                                                                                                                                                                   &       3 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL')                                                                                                                                                                          &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_RESTART', 'A\_RESTART', 'A\_ELICIT') &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY')                                                                                                                                                                            &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND')                                                                                                                                                                                                                               &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL')                                                                                                                                                                                                   &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL')                                                                                                                                                          &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL')                                                                                                                                  &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_RESTART', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_DENY')                                                                                                                                   &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS')                                                                                                                                                                                                                              &       2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_RECOMMEND')                                                                                                          &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL')                                                                                                                                                                                                                                              &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND')                                                                                                                                                            &       1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL')                                                                                                                                                                          &       1 \\ \hline
		\hline
		Total & 82 \\ \hline
	\end{tabularx}
\end{table}

\subsection{Dialogue of the Deaf}

\begin{table}
	\centering
	\caption{Dialogue of deaf summary.}
	\begin{tabularx}{\linewidth}{X|c}
		Sequence of intents &  Count \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_RESTART+REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_RESTART+REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_DENY', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_RESTART+REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_DENY', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_RESTART+REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_DENY', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_INQUIRE') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_ACCEPT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_RESTART', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_INQUIRE') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY', 'A\_INFORM', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		\hline
		Total & 20 \\ \hline
	\end{tabularx}
\end{table}


\section{Summary per failure for second iteration}

\subsection{System failure}

\begin{table}
	\centering
	\caption{System failure summary. The sign + is used to represent utterance with more than one intent.}
	\begin{tabularx}{\linewidth}{X|c}
		Sequence of intents &  Count \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL') & 4 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'A\_RESTART+ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM') & 1 \\ \hline
		\hline
		Total & 11 \\ \hline
	\end{tabularx}
\end{table}

\subsection{Flow discontinuation}

\begin{table}
	\centering
	\caption{Flow discontinuation summary.}
	\begin{tabularx}{\linewidth}{X|c}
		Sequence of intents &  Count \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL') & 3 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 10 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL') & 7 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_NO\_RESULTS') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL') & 4 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 4 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_NO\_RESULTS') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS') & 3 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_INQUIRE') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_DENY') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_DENY') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REMOVE\_PREFERENCE') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_RESTART', 'U\_REVEAL', 'A\_INFORM') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REMOVE\_PREFERENCE') & 1 \\ \hline
		\hline
		Total & 80 \\ \hline
	\end{tabularx}
\end{table}

\subsection{Dialogue of the Deaf}

\begin{table}
	\centering
	\caption{Dialogue of deaf summary.}
	\begin{tabularx}{\linewidth}{X|c}
		Sequence of intents &  Count \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_RESTART+REVEAL', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL') & 2 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_DENY', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS', 'U\_RESTART+REVEAL', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_NO\_RESULTS', 'U\_RESTART+REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT', 'A\_NO\_RESULTS', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_INQUIRE') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY', 'A\_INFORM', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY', 'A\_INFORM', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_DENY', 'A\_INFORM', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_WELCOME', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_ACCEPT', 'A\_CONTINUE\_RECOMMENDATION', 'U\_REJECT', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_REVEAL') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_CONTINUE\_RECOMMENDATION', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_RECOMMEND', 'U\_RESTART', 'A\_INFORM', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REVEAL', 'A\_ELICIT', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REVEAL', 'A\_NO\_RESULTS', 'U\_REJECT') & 1 \\ \hline
		('A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_WELCOME', 'U\_REVEAL', 'A\_COUNT\_RESULTS+ELICIT', 'U\_REVEAL', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REJECT', 'A\_RECOMMEND', 'U\_INQUIRE', 'A\_INFORM', 'U\_REMOVE\_PREFERENCE', 'A\_RECOMMEND', 'U\_ACCEPT', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_REVEAL', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION', 'A\_CANT\_HELP', 'U\_CONTINUE\_RECOMMENDATION') & 1 \\ \hline
		\hline
		Total & 26 \\ \hline
	\end{tabularx}
\end{table}

